Enhancing Column Generation by a Machine-Learning-Based Pricing Heuristic for Graph Coloring

Column Generation (CG) is an effective method for solving large-scale optimization problems. CG starts by solving a sub-problem with a subset of columns (i.e., variables) and gradually includes new columns that can improve the solution of the current subproblem. The new columns are generated as needed by repeatedly solving a pricing problem, which is often NP-hard and is a bottleneck of the CG approach. To tackle this, we propose a Machine-Learning-based Pricing Heuristic (MLPH)that can generate many high-quality columns efficiently. In each iteration of CG, our MLPH leverages an ML model to predict the optimal solution of the pricing problem, which is then used to guide a sampling method to efficiently generate multiple high-quality columns. Using the graph coloring problem, we empirically show that MLPH significantly enhancesCG as compared to six state-of-the-art methods, and the improvement in CG can lead to substantially better performance of the branch-and-price exact method.

==> data/cg/large-cs/table_cg.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccc@{}}
        \toprule
        C4000.5 & N/A & N/A & N/A & N/A & N/A & 46.4 & 16.4 & 55.9 & 50.9 & 95.6 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        wap03a & N/A & N/A & N/A & N/A & N/A & 21.1 & 7.0 & 25.0 & 24.0 & 32.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        C2000.5 & N/A & N/A & N/A & N/A & N/A & 220.1 & 62.1 & 229.4 & 188.8 & 583.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        ash958GPIA & N/A & N/A & N/A & N/A & N/A & 15.6 & 5.8 & 21.0 & 19.6 & 50.6 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        wap02a & N/A & N/A & N/A & N/A & N/A & 57.0 & 12.6 & 73.2 & 69.0 & 199.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        wap04a & N/A & N/A & N/A & N/A & N/A & 19.0 & 7.0 & 22.0 & 21.0 & 29.2 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        4-FullIns\_5 & N/A & N/A & N/A & N/A & N/A & 5.9 & 4.8 & 8.5 & 7.1 & 37.9 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        wap01a & 36.9 & N/A & 71.2 & N/A & N/A & N/A & 13.5 & 72.5 & 73.9 & 227.1 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/large-cs/table_rc.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccc@{}}
        \toprule
        C4000.5 & 186653.9 & 186593.9 & 186353.2 & 187108.4 & 185798.5 & -0.49 & -0.49 & -0.48 & -0.48 & -0.5 & -0.12 & -0.12 & -0.12 & -0.12 & -0.12 \\
        wap03a & 236681.9 & 236671.8 & 236684.0 & 236674.2 & 236675.8 & -2.42 & -2.42 & -2.42 & -2.42 & -2.44 & -1.8 & -1.81 & -1.79 & -1.81 & -1.81 \\
        C2000.5 & 89419.9 & 89443.6 & 89066.4 & 89406.4 & 88801.4 & -0.5 & -0.52 & -0.5 & -0.5 & -0.52 & -0.12 & -0.12 & -0.12 & -0.12 & -0.12 \\
        ash958GPIA & 95896.6 & 95895.5 & 95893.6 & 95898.4 & 95885.1 & -0.12 & -0.12 & -0.12 & -0.12 & -0.13 & -0.07 & -0.07 & -0.07 & -0.07 & -0.07 \\
        wap02a & 123313.0 & 123309.9 & 123308.1 & 123303.1 & 123314.1 & -1.75 & -1.73 & -1.74 & -1.74 & -1.74 & -1.19 & -1.19 & -1.2 & -1.2 & -1.19 \\
        wap04a & 205329.9 & 230718.4 & 195957.6 & 197376.0 & 199818.6 & -2.46 & -2.48 & -2.49 & -2.45 & -2.45 & -1.85 & -1.84 & -1.84 & -1.84 & -1.84 \\
        4-FullIns\_5 & 28705.8 & 33361.6 & 30465.8 & 28963.8 & 29165.9 & -4.35 & -4.35 & -4.34 & -4.34 & -4.35 & -3.06 & -3.05 & -3.05 & -3.06 & -3.04 \\
        wap01a & 118506.0 & 118505.5 & 118509.2 & 118502.5 & 118504.9 & -1.81 & -1.78 & -1.78 & -1.8 & -1.79 & -1.25 & -1.24 & -1.24 & -1.24 & -1.24 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/large-cs/table_solving_stats.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccc@{}}
        \toprule
        C4000.5 & 0 & 0 & 0 & 0 & 0 & 264.078 & 268.921 & 264.277 & 265.833 & 305.334 & 8078.9 & 8417.3 & 8130.6 & 8142.2 & 8038.0 \\
        wap03a & 0 & 0 & 0 & 0 & 0 & 45.121 & 46.793 & 45.684 & 45.827 & 73.366 & 8211.9 & 9390.9 & 8229.4 & 8128.0 & 8149.2 \\
        C2000.5 & 0 & 0 & 0 & 0 & 0 & 138.35 & 140.998 & 138.359 & 139.062 & 165.638 & 8017.0 & 8075.7 & 8024.3 & 8027.5 & 8006.6 \\
        ash958GPIA & 0 & 0 & 0 & 0 & 0 & 3.378 & 3.398 & 3.381 & 3.386 & 3.423 & 8353.0 & 9117.2 & 8337.6 & 8270.0 & 8083.1 \\
        wap02a & 0 & 0 & 0 & 0 & 0 & 40.039 & 41.063 & 40.217 & 40.552 & 54.388 & 8073.2 & 8432.4 & 8087.0 & 8091.6 & 8022.9 \\
        wap04a & 0 & 0 & 0 & 0 & 0 & 44.751 & 46.281 & 45.112 & 45.267 & 78.609 & 8398.3 & 9953.6 & 8220.6 & 8087.9 & 8132.9 \\
        4-FullIns\_5 & 0 & 0 & 0 & 0 & 0 & 6.692 & 6.568 & 6.662 & 6.632 & 10.036 & 9404.2 & 9441.3 & 8561.3 & 8795.6 & 8077.1 \\
        wap01a & 8 & 0 & 6 & 0 & 0 & 41.0 & 41.664 & 41.0 & 41.283 & 52.981 & 4321.3 & 8445.7 & 7790.0 & 8054.0 & 8010.2 \\
        statistic & 8 & 0 & 6 & 0 & 0 & 37.189 & 37.835 & 37.294 & 37.435 & 49.765 & 7690.9 & 8888.2 & 8169.8 & 8196.3 & 8064.8 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/large/table_cg.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccc@{}}
        \toprule
        C4000.5 & N/A & N/A & N/A & N/A & N/A & 56.1 & 30.7 & 24.0 & 20.7 & 68.9 & 1.0 & 1.0 & 0.95 & 0.61 & 1.0 \\
        wap03a & N/A & N/A & N/A & N/A & N/A & 23.8 & 30.4 & 33.2 & 33.5 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.0 \\
        C2000.5 & N/A & N/A & N/A & N/A & N/A & 259.3 & 47.3 & 49.7 & 49.5 & 149.5 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        ash958GPIA & N/A & N/A & N/A & N/A & N/A & 18.8 & 23.0 & 28.7 & 23.5 & 28.8 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 \\
        wap02a & 68.0 & N/A & N/A & N/A & N/A & 66.8 & 46.9 & 106.8 & 42.7 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.0 \\
        wap04a & N/A & N/A & N/A & N/A & N/A & 21.1 & 26.6 & 29.7 & 30.7 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.0 \\
        4-FullIns\_5 & N/A & N/A & N/A & N/A & N/A & 6.8 & 9.0 & 9.8 & 12.0 & 9.3 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        wap01a & 36.5 & N/A & N/A & N/A & N/A & N/A & 47.6 & 99.2 & 43.7 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.02 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/large/table_rc.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}ccccccccccc@{}}
        \toprule
        C4000.5 & 185611.9 & 140979.4 & 2.4 & 1.1 & 89.8 & -0.49 & -0.39 & -0.24 & -0.15 & -0.3 \\
        wap03a & 234610.1 & 277.8 & 5.8 & 42.1 & 0.0 & -2.44 & -0.35 & -3.05 & -3.04 & 0.0 \\
        C2000.5 & 89512.1 & 91193.0 & 1.9 & 1.7 & 253.5 & -0.5 & -0.42 & -0.23 & -0.23 & -0.38\\
        ash958GPIA & 95888.6 & 1962.9 & 29.1 & 1507.0 & 58.0 & -0.12 & -0.05 & -0.2 & -0.2 & -0.06 \\
        wap02a & 123309.2 & 202.7 & 10.8 & 1064.8 & 0.0 & -1.76 & -0.33 & -2.3 & -2.29 & 0.0 \\
        wap04a & 191494.5 & 277.8 & 5.5 & 23.0 & 0.0 & -2.48 & -0.37 & -3.11 & -2.94 & 0.0 \\
        4-FullIns\_5 & 28273.2 & 26.3 & 3.0 & 4820.1 & 676.8 & -4.37 & -0.55 & -4.37 & -4.38 & -3.93 \\
        wap01a & 118508.7 & 243.0 & 10.6 & 1132.1 & 0.0 & -1.79 & -0.36 & -2.32 & -2.33 & -0.0\\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/large/table_solving_stats.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}ccccccc@{}}
        \toprule
        C4000.5  & 0 & 263.474 & 264.545 & 304.798 & 304.894 & 286.648 \\
        wap03a  & 0 & 44.867 & 70.091 & 54.094 & 54.495 & 76.044 \\
        C2000.5  & 0 & 137.908 & 140.78 & 164.596 & 164.624 & 141.977 \\
        ash958GPIA  & 0 & 3.37 & 3.366 & 3.426 & 3.424 & 3.405 \\
        wap02a & 3  & 40.021 & 58.569 & 42.687 & 43.494 & 64.515 \\
        wap04a  & 0 & 44.453 & 75.067 & 55.999 & 55.463 & 81.131 \\
        4-FullIns\_5  & 0 & 6.683 & 12.315 & 9.601 & 7.673 & 7.91 \\
        wap01a & 24  & 41.0 & 56.212 & 42.707 & 43.343 & 62.128 \\
        statistic & 27  & 37.089 & 49.201 & 43.077 & 42.15 & 49.492 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/small/table_cg.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccccccccc@{}}
        \toprule
        ash608GPIA & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 5.4 & 6.7 & 8.9 & 8.2 & 7.2 & 6.8 & 6.8 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.92 & 0.83 \\
        wap08a & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 4.7 & 8.8 & 9.0 & 9.2 & 5.2 & 1.3 & 10.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 & 0.13 & 1.0 \\
        wap07a & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 4.9 & 8.5 & 7.7 & 8.5 & 5.5 & 2.1 & 9.5 & 1.0 & 1.0 & 1.0 & 1.0 & 0.93 & 0.32 & 1.0 \\
        abb313GPIA & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 6.4 & 9.1 & 11.8 & 11.4 & 9.1 & 9.2 & 8.5 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.79 \\
        3-FullIns\_5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 10.5 & 12.2 & 13.3 & 13.7 & 7.8 & 11.7 & 14.5 & 1.0 & 1.0 & 1.0 & 1.0 & 0.01 & 1.0 & 0.53 \\
        DSJC1000.1 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 9.9 & 9.4 & 14.0 & 12.9 & 7.1 & 11.8 & 18.9 & 1.0 & 1.0 & 1.0 & 1.0 & 0.84 & 1.0 & 1.0 \\
        3-Insertions\_5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 9.5 & 17.1 & 19.4 & 12.9 & 11.0 & 9.5 & 18.7 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.72 \\
        r1000.1 & 2.1 & 2.7 & 3.2 & 2.8 & 7.6 & 6.0 & 5.8 & N/A & N/A & N/A & N/A & 13.8 & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        DSJC1000.5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 23.8 & 16.1 & 21.8 & 20.0 & 22.9 & 17.5 & 38.2 & 1.0 & 1.0 & 0.97 & 0.95 & 1.0 & 0.96 & 1.0 \\
        flat1000\_60\_0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 22.4 & 17.8 & 21.5 & 20.4 & 20.5 & 20.5 & 40.6 & 1.0 & 1.0 & 0.97 & 0.95 & 1.0 & 0.97 & 1.0 \\
        flat1000\_76\_0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 23.2 & 18.1 & 21.1 & 20.2 & 21.0 & 19.4 & 40.0 & 1.0 & 1.0 & 0.96 & 0.93 & 1.0 & 0.98 & 1.0 \\
        flat1000\_50\_0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 37.9 & 21.0 & 22.5 & 22.6 & 20.1 & 25.7 & 44.8 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 1.0 & 1.0 \\
        5-FullIns\_4 & 17.7 & N/A & N/A & 26.0 & N/A & N/A & N/A & 26.9 & 32.6 & 49.9 & 33.5 & 17.1 & 29.5 & 60.9 & 0.65 & 0.97 & 1.0 & 1.0 & 0.88 & 1.0 & 0.48 \\
        will199GPIA & 14.0 & N/A & 78.8 & 28.6 & N/A & N/A & N/A & 49.0 & 30.8 & 84.2 & 31.9 & 17.8 & 30.0 & 43.0 & 0.99 & 1.0 & 1.0 & 1.0 & 0.96 & 1.0 & 0.92 \\
        wap05a & 2.1 & N/A & 9.4 & 6.7 & 7.2 & N/A & N/A & N/A & 33.0 & N/A & N/A & N/A & 30.7 & 90.8 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 & 1.0 \\
        wap06a & 17.5 & N/A & N/A & N/A & N/A & N/A & N/A & 19.4 & 34.5 & 40.5 & 29.1 & 23.9 & 20.9 & 90.2 & 0.99 & 1.0 & 1.0 & 1.0 & 1.0 & 0.66 & 0.98 \\
        DSJC1000.9 & 20.6 & 8.7 & N/A & N/A & 148.9 & N/A & N/A & N/A & N/A & 45.0 & 45.0 & N/A & 145.7 & 186.2 & 0.93 & 0.96 & 0.43 & 0.38 & 1.0 & 1.0 & 1.0 \\
        DSJC500.1 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 86.5 & 39.9 & 46.8 & 46.2 & 13.3 & 41.6 & 221.3 & 1.0 & 1.0 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0 \\
        2-FullIns\_5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 36.6 & 48.3 & 131.4 & 40.1 & 43.7 & 42.0 & 212.8 & 0.91 & 0.95 & 1.0 & 1.0 & 1.0 & 0.99 & 0.49 \\
        4-Insertions\_4 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 44.0 & 40.7 & 136.9 & 37.7 & 33.5 & 36.2 & 250.9 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        2-Insertions\_5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 32.5 & 49.1 & 104.7 & 39.3 & 34.1 & 34.3 & 281.2 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.93 \\
        4-FullIns\_4 & 18.2 & N/A & 104.9 & 37.4 & N/A & 26.6 & N/A & N/A & 50.2 & N/A & 46.3 & 38.3 & 55.5 & 278.6 & 0.81 & 0.9 & 1.0 & 1.0 & 0.98 & 0.96 & 0.33 \\
        r1000.5 & 48.4 & 23.7 & N/A & N/A & 79.8 & N/A & N/A & 58.3 & N/A & 51.9 & 51.9 & N/A & 52.1 & 291.9 & 1.0 & 1.0 & 0.86 & 0.86 & 1.0 & 0.91 & 1.0 \\
        DSJC500.5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 164.8 & 47.0 & 48.0 & 47.6 & 156.3 & 133.8 & 448.4 & 0.99 & 1.0 & 0.25 & 0.14 & 1.0 & 0.68 & 1.0 \\
        1-Insertions\_6 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 38.3 & 52.2 & 74.3 & 45.7 & 44.5 & 38.2 & 357.9 & 1.0 & 0.99 & 1.0 & 1.0 & 1.0 & 1.0 & 0.65 \\
        le450\_5a & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 82.2 & 48.7 & 51.8 & 47.1 & 23.2 & 53.3 & 353.5 & 1.0 & 0.99 & 1.0 & 1.0 & 0.95 & 1.0 & 1.0 \\
        le450\_5b & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 87.4 & 47.3 & 52.5 & 48.0 & 28.1 & 51.6 & 380.9 & 1.0 & 0.99 & 1.0 & 1.0 & 0.96 & 1.0 & 1.0 \\
        r1000.1c & 4.0 & 3.9 & N/A & N/A & 20.7 & 11.5 & 623.0 & N/A & N/A & 55.0 & 55.0 & N/A & N/A & 635.4 & 1.0 & 1.0 & 0.22 & 0.2 & 1.0 & 0.99 & 0.07 \\
        le450\_25a & 2.0 & 2.8 & 3.7 & 4.7 & 3.0 & 22.5 & 38.2 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.97 \\
        le450\_15d & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 130.1 & 51.9 & 53.9 & 49.1 & 44.2 & 78.2 & 425.7 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.96 & 0.96 \\
        le450\_15c & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 126.5 & 52.0 & 53.9 & 49.2 & 42.4 & 76.1 & 449.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.98 & 0.98 & 0.97 \\
        le450\_15b & 10.0 & N/A & 131.2 & 22.7 & N/A & N/A & N/A & N/A & 53.1 & N/A & N/A & 34.8 & 70.7 & 530.6 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.92 \\
        le450\_15a & 11.5 & N/A & 139.8 & 23.3 & N/A & N/A & N/A & N/A & 53.5 & N/A & N/A & 35.0 & 70.2 & 553.2 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.92 \\
        le450\_25c & 20.6 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 53.6 & 90.9 & 45.8 & 48.0 & 81.8 & 633.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.82 \\
        le450\_25d & 17.0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 53.0 & 87.4 & 46.2 & 46.8 & 80.9 & 652.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.83 \\
        le450\_5c & N/A & 18.0 & N/A & N/A & N/A & N/A & N/A & 175.6 & 50.4 & 60.5 & 54.1 & 44.5 & 60.3 & 792.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        queen16\_16 & 12.3 & 15.0 & 86.4 & 15.8 & N/A & 54.5 & 418.5 & N/A & N/A & N/A & N/A & 41.0 & 40.9 & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.91 & 1.0 \\
        le450\_5d & N/A & 21.8 & N/A & N/A & N/A & N/A & N/A & 185.6 & 51.7 & 60.1 & 54.2 & 42.8 & 60.6 & 817.3 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        DSJC500.9 & 6.6 & 5.7 & N/A & N/A & 47.5 & 63.8 & 284.5 & N/A & N/A & 58.0 & 58.0 & N/A & N/A & N/A & 0.99 & 0.99 & 0.17 & 0.23 & 1.0 & 1.0 & 0.95 \\
        3-FullIns\_4 & 8.4 & 16.8 & 60.7 & 23.9 & 44.1 & 12.2 & 406.3 & N/A & N/A & N/A & N/A & N/A & N/A & 1021.0 & 0.88 & 0.88 & 1.0 & 1.0 & 1.0 & 0.99 & 0.41 \\
        3-Insertions\_4 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 85.4 & 48.0 & 343.0 & 51.2 & 60.2 & 94.6 & 878.8 & 0.96 & 0.97 & 1.0 & 1.0 & 1.0 & 1.0 & 0.96 \\
        queen15\_15 & 10.4 & 12.6 & 79.5 & 12.8 & N/A & 44.8 & 356.7 & N/A & N/A & N/A & N/A & 41.5 & 65.0 & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.93 & 1.0 \\
        school1 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 249.1 & 57.1 & 84.9 & 57.0 & 403.3 & 271.2 & 1428.2 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.9 & 0.88 \\
        flat300\_26\_0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 426.4 & 140.6 & 59.0 & 58.5 & 936.8 & 1199.5 & 2379.3 & 1.0 & 1.0 & 1.0 & 0.92 & 1.0 & 0.25 & 1.0 \\
        flat300\_28\_0 & N/A & 111.2 & N/A & N/A & 124.5 & 280.2 & 1144.0 & 627.7 & 135.9 & 59.0 & 58.6 & N/A & 974.6 & 1304.5 & 0.25 & 0.58 & 0.98 & 0.93 & 1.0 & 0.62 & 0.69 \\
        DSJR500.5 & 7.3 & 5.0 & N/A & N/A & 28.1 & 100.5 & 196.0 & N/A & N/A & 58.3 & 58.2 & N/A & 964.0 & N/A & 1.0 & 1.0 & 0.55 & 0.41 & 1.0 & 0.59 & 1.0 \\
        school1\_nsh & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 315.2 & 57.1 & 90.3 & 57.0 & 431.7 & 604.4 & 1539.5 & 0.97 & 1.0 & 1.0 & 1.0 & 1.0 & 0.52 & 0.85 \\
        flat300\_20\_0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 404.0 & 137.9 & 59.0 & 58.9 & 1070.5 & 1630.0 & 2808.2 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 0.38 & 0.99 \\
        DSJC250.1 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 110.5 & 85.4 & 58.4 & 58.0 & 42.6 & 268.8 & 552.0 & 0.99 & 0.99 & 1.0 & 1.0 & 0.97 & 1.0 & 0.99 \\
        queen14\_14 & 10.0 & 10.9 & 76.7 & 11.1 & 20.5 & 51.1 & 312.7 & N/A & N/A & N/A & N/A & N/A & 283.0 & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.9 & 1.0 \\
        DSJC250.5 & 1025.0 & 65.7 & N/A & N/A & 96.3 & 154.3 & 1294.6 & 1209.1 & N/A & 54.8 & 59.0 & N/A & N/A & 2109.0 & 0.12 & 0.67 & 1.0 & 1.0 & 1.0 & 0.85 & 0.46 \\
        queen13\_13 & 7.5 & 7.9 & 61.9 & 8.0 & 18.8 & 31.9 & 237.5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        DSJR500.1c & 2.0 & 2.0 & 12.5 & 20.8 & 2.8 & 2.5 & 56.2 & N/A & N/A & 59.8 & 60.2 & N/A & N/A & N/A & 0.83 & 0.83 & 0.04 & 0.03 & 0.83 & 0.83 & 0.15 \\
        1-FullIns\_5 & 5.9 & 34.0 & 534.4 & N/A & N/A & 16.3 & N/A & N/A & 59.0 & 607.0 & 56.0 & 341.2 & N/A & 2135.8 & 1.0 & 0.64 & 1.0 & 1.0 & 1.0 & 0.98 & 0.56 \\
        1-Insertions\_5 & N/A & N/A & N/A & N/A & N/A & 102.0 & N/A & 581.9 & 83.0 & 416.6 & 56.0 & 356.6 & N/A & 2146.1 & 0.42 & 0.96 & 1.0 & 1.0 & 1.0 & 1.0 & 0.76 \\
        queen12\_12 & 7.3 & 7.2 & 59.4 & 7.2 & 19.5 & 32.0 & 211.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        2-FullIns\_4 & 4.8 & 7.0 & 28.2 & 12.5 & 24.6 & 5.7 & 672.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 0.98 & 1.0 & 1.0 & 1.0 & 1.0 & 0.49 \\
        DSJC250.9 & 4.8 & 4.9 & N/A & N/A & 18.7 & 21.9 & 66.0 & N/A & N/A & 28.6 & 27.1 & N/A & N/A & N/A & 1.0 & 1.0 & 0.15 & 0.17 & 1.0 & 1.0 & 1.0 \\
        2-Insertions\_4 & N/A & N/A & 308.7 & N/A & 225.2 & 105.2 & N/A & 866.1 & 239.9 & N/A & 57.0 & N/A & N/A & 2648.2 & 0.33 & 0.61 & 1.0 & 1.0 & 1.0 & 0.98 & 0.79 \\
        r250.5 & 5.0 & 4.5 & 34.7 & 7.1 & 16.2 & 115.9 & 89.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.88 & 1.0 \\
        queen11\_11 & 7.0 & 6.4 & 53.6 & 6.0 & 21.3 & 27.1 & 176.4 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        mug100\_1 & 17.2 & 23.7 & 50.8 & N/A & 29.0 & 70.8 & 214.3 & N/A & N/A & N/A & 58.3 & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        mug100\_25 & 13.2 & 19.4 & 45.0 & 53.0 & 24.8 & 64.1 & 193.5 & N/A & N/A & N/A & 58.9 & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        mug88\_1 & 10.4 & 13.5 & 33.2 & 49.4 & 18.4 & 49.8 & 120.2 & N/A & N/A & N/A & 60.4 & N/A & N/A & N/A & 1.0 & 0.98 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        myciel7 & 178.3 & N/A & 412.5 & N/A & 465.6 & 57.2 & N/A & N/A & 131.8 & N/A & 58.0 & 487.8 & N/A & 3554.1 & 0.36 & 0.47 & 1.0 & 1.0 & 1.0 & 1.0 & 0.36 \\
        DSJC125.1 & N/A & N/A & 172.7 & N/A & 92.9 & N/A & N/A & 1692.1 & 841.2 & N/A & 59.0 & N/A & 1487.1 & 3553.4 & 0.18 & 0.36 & 1.0 & 1.0 & 1.0 & 0.35 & 0.37 \\
        mug88\_25 & 11.9 & 13.6 & 38.1 & 50.8 & 21.6 & 46.3 & 148.3 & N/A & N/A & N/A & 59.3 & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        queen10\_10 & 6.5 & 5.4 & 52.8 & 5.2 & 25.2 & 27.2 & 175.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        DSJC125.5 & 283.8 & 16.2 & 51.6 & 33.3 & 40.3 & 50.7 & 412.4 & N/A & N/A & N/A & 60.3 & N/A & N/A & N/A & 0.2 & 0.85 & 1.0 & 0.57 & 1.0 & 0.99 & 0.64 \\
        4-Insertions\_3 & 1154.5 & 422.8 & 83.5 & 29.0 & 48.4 & 58.2 & 513.0 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.08 & 0.11 & 1.0 & 1.0 & 1.0 & 0.94 & 0.73 \\
        queen9\_9 & 5.6 & 4.5 & 35.6 & 4.4 & 18.5 & 21.1 & 105.5 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 \\
        r125.5 & 2.4 & 2.4 & 6.1 & 2.6 & 4.4 & 4.5 & 12.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 \\
        DSJC125.9 & 2.9 & 2.9 & 4.8 & 3.8 & 4.8 & 5.3 & 7.6 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 0.99 & 1.0 & 1.0 & 1.0 \\
        1-FullIns\_4 & 1.9 & 1.9 & 14.8 & 2.3 & 15.0 & 2.1 & 23.2 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.88 & 0.88 & 0.88 & 0.88 & 0.87 & 0.88 & 0.65 \\
        1-Insertions\_4 & 31.7 & 115.6 & 42.5 & 16.0 & 34.6 & 22.8 & 311.7 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.59 & 0.22 & 1.0 & 1.0 & 1.0 & 1.0 & 0.6 \\
        myciel6 & 15.3 & 628.8 & 92.9 & 26.0 & 85.0 & 29.9 & 934.4 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.64 & 0.06 & 1.0 & 1.0 & 1.0 & 1.0 & 0.32 \\
        3-Insertions\_3 & 75.6 & 73.0 & 33.5 & 10.0 & 22.9 & 28.1 & 255.6 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.32 & 0.29 & 1.0 & 1.0 & 1.0 & 1.0 & 0.51 \\
        queen8\_8 & 2.1 & 2.0 & 5.4 & 2.0 & 4.0 & 4.0 & 9.9 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        2-Insertions\_3 & 7.6 & 6.6 & 10.6 & 3.8 & 9.4 & 10.2 & 27.9 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.83 & 0.82 & 1.0 & 1.0 & 1.0 & 1.0 & 0.79 \\
        myciel5 & 4.4 & 19.2 & 14.3 & 4.6 & 12.7 & 12.4 & 74.6 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.97 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.55 \\
        myciel4 & 2.0 & 2.0 & 2.8 & 2.0 & 3.0 & 2.8 & 3.8 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & 0.83 & 0.81 & 0.83 & 0.83 & 0.83 & 0.83 & 0.76 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/small/table_rc.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccccccccc@{}}
        \toprule
        ash608GPIA & 15254.2 & 277.1 & 26.9 & 438.7 & 4695.6 & 22.3 & 0.9 & -0.11 & -0.05 & -0.18 & -0.18 & -0.11 & -0.06 & -0.02 & -0.06 & -0.01 & -0.13 & -0.08 & -0.07 & -0.02 & -0.02 \\
        wap08a & 57150.2 & 206.5 & 3.8 & 6.5 & 509.2 & 0.2 & 1.0 & -1.59 & -0.37 & -1.69 & -1.91 & -0.56 & -0.01 & -0.55 & -0.99 & -0.07 & -1.17 & -1.13 & -0.27 & -0.01 & -0.55 \\
        wap07a & 63284.2 & 249.2 & 3.2 & 6.1 & 493.2 & 0.7 & 1.0 & -1.55 & -0.37 & -1.47 & -1.83 & -0.59 & -0.02 & -0.75 & -0.98 & -0.07 & -1.0 & -1.1 & -0.28 & -0.02 & -0.75 \\
        abb313GPIA & 26178.0 & 142.2 & 13.2 & 321.3 & 1734.8 & 41.0 & 0.9 & -0.45 & -0.16 & -0.63 & -0.63 & -0.46 & -0.23 & -0.16 & -0.19 & -0.03 & -0.44 & -0.32 & -0.27 & -0.06 & -0.16 \\
        3-FullIns\_5 & 5738.9 & 9.5 & 3.0 & 1164.9 & 0.0 & 502.4 & 0.6 & -2.62 & -0.41 & -2.63 & -2.63 & 0.0 & -2.44 & -0.33 & -1.66 & -0.14 & -2.16 & -2.32 & 0.0 & -0.76 & -0.33 \\
        DSJC1000.1 & 50057.5 & 2319.8 & 2.9 & 2.5 & 107.0 & 440.2 & 1.0 & -0.58 & -0.25 & -0.27 & -0.27 & -0.14 & -0.45 & -0.46 & -0.24 & -0.04 & -0.16 & -0.17 & -0.07 & -0.09 & -0.46 \\
        3-Insertions\_5 & 17041.5 & 22.2 & 2.0 & 5128.4 & 5793.0 & 828.8 & 0.8 & -3.19 & -0.38 & -3.24 & -3.24 & -2.22 & -3.0 & -0.18 & -2.88 & -0.1 & -2.84 & -2.38 & -1.12 & -1.33 & -0.18 \\
        r1000.1 & 50030.5 & 1159.0 & 7.3 & 2892.4 & 1749.4 & 52.2 & 1.0 & -0.5 & -0.17 & -0.7 & -0.7 & -0.51 & -0.22 & -0.49 & -0.25 & -0.03 & -0.36 & -0.35 & -0.26 & -0.05 & -0.49 \\
        DSJC1000.5 & 37906.0 & 26552.0 & 2.0 & 1.7 & 23.5 & 298.2 & 1.0 & -0.49 & -0.41 & -0.17 & -0.16 & -0.4 & -0.43 & -0.45 & -0.1 & -0.06 & -0.13 & -0.13 & -0.21 & -0.07 & -0.45 \\
        flat1000\_60\_0 & 34218.0 & 32003.5 & 1.6 & 1.5 & 21.7 & 412.5 & 1.0 & -0.49 & -0.49 & -0.16 & -0.16 & -0.39 & -0.45 & -0.51 & -0.09 & -0.06 & -0.14 & -0.15 & -0.2 & -0.06 & -0.51 \\
        flat1000\_76\_0 & 35215.0 & 33548.5 & 1.4 & 1.4 & 23.0 & 401.1 & 1.0 & -0.46 & -0.42 & -0.18 & -0.19 & -0.4 & -0.45 & -0.45 & -0.09 & -0.06 & -0.16 & -0.17 & -0.21 & -0.06 & -0.45 \\
        flat1000\_50\_0 & 32684.0 & 19579.7 & 1.6 & 1.5 & 25.6 & 236.0 & 1.0 & -0.72 & -0.87 & -0.22 & -0.21 & -0.44 & -0.65 & -0.59 & -0.09 & -0.06 & -0.17 & -0.18 & -0.22 & -0.07 & -0.59 \\
        5-FullIns\_4 & 17277.5 & 32.0 & 3.6 & 4770.3 & 449.9 & 337.1 & 0.6 & -0.92 & -0.24 & -0.96 & -0.96 & -0.96 & -0.77 & -0.12 & -0.43 & -0.06 & -0.76 & -0.94 & -0.47 & -0.12 & -0.12 \\
        will199GPIA & 35012.4 & 615.0 & 7.3 & 8904.2 & 1290.8 & 151.2 & 1.0 & -0.5 & -0.19 & -0.57 & -0.57 & -0.48 & -0.36 & -0.17 & -0.25 & -0.04 & -0.33 & -0.49 & -0.24 & -0.08 & -0.17 \\
        wap05a & 45304.6 & 291.7 & 8.0 & 214.0 & 401.3 & 2.2 & 1.0 & -1.14 & -0.39 & -1.4 & -1.37 & -1.3 & -0.11 & -0.55 & -0.59 & -0.07 & -1.12 & -0.72 & -0.51 & -0.08 & -0.55 \\
        wap06a & 47401.9 & 231.3 & 7.7 & 207.0 & 385.2 & 1.8 & 1.0 & -1.21 & -0.37 & -1.44 & -1.42 & -1.3 & -0.06 & -0.53 & -0.64 & -0.07 & -1.21 & -0.74 & -0.55 & -0.04 & -0.53 \\
        DSJC1000.9 & 2239.2 & 4207.4 & 1.3 & 1.3 & 11.1 & 12.5 & 1.0 & -0.4 & -0.41 & -0.1 & -0.11 & -0.41 & -0.4 & -0.39 & -0.05 & -0.05 & -0.08 & -0.09 & -0.21 & -0.16 & -0.39 \\
        DSJC500.1 & 25029.4 & 1888.5 & 10.2 & 26.6 & 169.2 & 2463.9 & 1.0 & -0.64 & -0.29 & -0.55 & -0.55 & -0.32 & -0.56 & -0.39 & -0.28 & -0.05 & -0.33 & -0.17 & -0.15 & -0.09 & -0.39 \\
        2-FullIns\_5 & 28020.0 & 58.8 & 2.8 & 5427.5 & 410.6 & 1643.5 & 0.7 & -1.37 & -0.45 & -1.38 & -1.38 & -1.38 & -0.94 & -0.13 & -0.81 & -0.1 & -1.18 & -1.32 & -0.71 & -0.41 & -0.13 \\
        4-Insertions\_4 & 21038.5 & 5408.3 & 2.4 & 17811.8 & 2015.5 & 18527.9 & 1.0 & -0.89 & -0.39 & -0.95 & -0.95 & -0.76 & -0.93 & -0.3 & -0.72 & -0.06 & -0.67 & -0.6 & -0.4 & -0.57 & -0.3 \\
        2-Insertions\_5 & 22637.8 & 187.1 & 2.2 & 11643.6 & 2397.5 & 14467.7 & 1.0 & -1.84 & -0.46 & -1.85 & -1.85 & -1.85 & -1.85 & -0.25 & -1.4 & -0.07 & -1.27 & -1.28 & -0.89 & -1.13 & -0.25 \\
        4-FullIns\_4 & 27861.5 & 244.4 & 3.2 & 11288.0 & 272.7 & 377.7 & 0.6 & -0.6 & -0.27 & -0.63 & -0.63 & -0.63 & -0.57 & -0.14 & -0.27 & -0.06 & -0.46 & -0.61 & -0.31 & -0.1 & -0.14 \\
        r1000.5 & 16634.6 & 13192.6 & 1.9 & 1.7 & 34.8 & 116.5 & 1.0 & -0.6 & -0.5 & -0.25 & -0.26 & -0.67 & -0.45 & -0.55 & -0.12 & -0.08 & -0.2 & -0.21 & -0.34 & -0.08 & -0.55 \\
        DSJC500.5 & 12686.2 & 10771.2 & 2.0 & 2.1 & 23.3 & 302.7 & 1.0 & -0.44 & -0.4 & -0.22 & -0.21 & -0.46 & -0.45 & -0.42 & -0.1 & -0.06 & -0.19 & -0.18 & -0.24 & -0.07 & -0.42 \\
        1-Insertions\_6 & 16322.5 & 73.6 & 2.4 & 7568.8 & 1239.3 & 10858.0 & 0.7 & -2.36 & -0.48 & -2.36 & -2.36 & -2.36 & -2.36 & -0.13 & -1.51 & -0.08 & -1.55 & -1.69 & -1.11 & -0.94 & -0.13 \\
        le450\_5a & 22526.3 & 12282.5 & 16.7 & 2089.0 & 474.0 & 2643.7 & 1.0 & -1.01 & -0.7 & -1.23 & -1.22 & -0.62 & -1.03 & -0.6 & -0.47 & -0.22 & -0.72 & -0.47 & -0.3 & -0.15 & -0.6 \\
        le450\_5b & 22527.8 & 12263.1 & 16.4 & 1630.8 & 481.0 & 2720.1 & 1.0 & -0.97 & -0.64 & -1.2 & -1.2 & -0.58 & -1.07 & -0.54 & -0.43 & -0.2 & -0.64 & -0.4 & -0.28 & -0.17 & -0.54 \\
        r1000.1c & 23.9 & 24.0 & 0.3 & 0.2 & 9.6 & 4.0 & 0.2 & -0.3 & -0.3 & -0.05 & -0.02 & -0.3 & -0.3 & -0.04 & -0.09 & -0.09 & -0.05 & -0.02 & -0.14 & -0.2 & -0.04 \\
        le450\_25a & 22515.0 & 405.4 & 6.9 & 8886.5 & 209.6 & 14.7 & 1.0 & -0.67 & -0.27 & -0.72 & -0.72 & -0.72 & -0.28 & -0.28 & -0.33 & -0.05 & -0.46 & -0.69 & -0.3 & -0.1 & -0.28 \\
        le450\_15d & 22474.0 & 766.8 & 10.8 & 366.9 & 180.8 & 105.2 & 1.0 & -1.09 & -0.43 & -1.13 & -1.11 & -1.17 & -0.61 & -0.47 & -0.55 & -0.07 & -0.71 & -0.33 & -0.49 & -0.11 & -0.47 \\
        le450\_15c & 22496.5 & 740.5 & 11.1 & 385.7 & 164.7 & 126.9 & 1.0 & -1.09 & -0.42 & -1.12 & -1.13 & -1.17 & -0.63 & -0.45 & -0.55 & -0.07 & -0.71 & -0.35 & -0.49 & -0.11 & -0.45 \\
        le450\_15b & 22523.9 & 227.6 & 11.2 & 3345.6 & 291.1 & 49.7 & 1.0 & -1.03 & -0.32 & -1.16 & -1.16 & -1.16 & -0.46 & -0.54 & -0.57 & -0.07 & -0.8 & -0.5 & -0.47 & -0.1 & -0.54 \\
        le450\_15a & 22523.9 & 247.5 & 10.8 & 3329.4 & 290.8 & 68.3 & 1.0 & -1.07 & -0.34 & -1.18 & -1.18 & -1.18 & -0.5 & -0.51 & -0.58 & -0.07 & -0.81 & -0.51 & -0.47 & -0.1 & -0.51 \\
        le450\_25c & 22429.9 & 541.1 & 10.0 & 767.9 & 129.0 & 28.0 & 1.0 & -1.02 & -0.41 & -1.06 & -1.05 & -1.06 & -0.46 & -0.42 & -0.52 & -0.07 & -0.67 & -0.35 & -0.44 & -0.13 & -0.42 \\
        le450\_25d & 22423.7 & 690.7 & 9.7 & 882.8 & 133.6 & 32.2 & 1.0 & -0.98 & -0.39 & -1.03 & -1.01 & -1.03 & -0.47 & -0.34 & -0.49 & -0.07 & -0.69 & -0.37 & -0.43 & -0.12 & -0.34 \\
        le450\_5c & 22504.5 & 27218.2 & 10.5 & 4451.0 & 420.9 & 4385.6 & 1.0 & -1.33 & -1.25 & -1.43 & -1.43 & -1.43 & -1.42 & -0.73 & -0.48 & -0.44 & -0.73 & -1.07 & -1.12 & -0.35 & -0.73 \\
        queen16\_16 & 7207.5 & 13696.4 & 9.9 & 1588.5 & 27.6 & 112.9 & 1.0 & -0.23 & -0.26 & -0.3 & -0.3 & -0.27 & -0.24 & -0.26 & -0.05 & -0.05 & -0.21 & -0.1 & -0.14 & -0.04 & -0.26 \\
        le450\_5d & 22511.0 & 28603.0 & 13.0 & 4793.6 & 851.1 & 4660.2 & 1.0 & -1.3 & -1.27 & -1.39 & -1.39 & -1.39 & -1.37 & -0.75 & -0.47 & -0.42 & -0.77 & -1.11 & -0.72 & -0.32 & -0.75 \\
        DSJC500.9 & 437.2 & 489.9 & 0.5 & 0.5 & 7.7 & 8.3 & 1.0 & -0.41 & -0.41 & -0.04 & -0.06 & -0.39 & -0.41 & -0.41 & -0.07 & -0.07 & -0.04 & -0.06 & -0.21 & -0.19 & -0.41 \\
        3-FullIns\_4 & 13700.9 & 1340.0 & 3.8 & 21490.0 & 124.0 & 264.1 & 0.8 & -0.44 & -0.3 & -0.45 & -0.45 & -0.45 & -0.42 & -0.13 & -0.17 & -0.07 & -0.35 & -0.45 & -0.23 & -0.08 & -0.13 \\
        3-Insertions\_4 & 8786.8 & 16248.0 & 2.6 & 24684.9 & 1159.6 & 7718.2 & 1.0 & -0.73 & -0.39 & -0.77 & -0.77 & -0.77 & -0.75 & -0.31 & -0.49 & -0.06 & -0.52 & -0.55 & -0.38 & -0.36 & -0.31 \\
        queen15\_15 & 5518.4 & 10581.1 & 9.9 & 1706.4 & 28.8 & 93.3 & 1.0 & -0.22 & -0.25 & -0.28 & -0.28 & -0.28 & -0.22 & -0.25 & -0.05 & -0.05 & -0.18 & -0.09 & -0.15 & -0.04 & -0.25 \\
        school1 & 18433.2 & 1238.4 & 5.9 & 470.4 & 140.0 & 47.5 & 1.0 & -1.6 & -1.12 & -1.76 & -1.76 & -1.76 & -1.49 & -0.58 & -0.44 & -0.13 & -1.11 & -0.88 & -0.85 & -0.28 & -0.58 \\
        flat300\_26\_0 & 4947.5 & 4167.2 & 3.6 & 7.1 & 19.9 & 139.9 & 1.0 & -0.44 & -0.41 & -0.23 & -0.18 & -0.45 & -0.43 & -0.4 & -0.08 & -0.06 & -0.16 & -0.09 & -0.22 & -0.08 & -0.4 \\
        flat300\_28\_0 & 5200.3 & 5116.8 & 4.5 & 4.3 & 18.6 & 158.6 & 1.0 & -0.42 & -0.39 & -0.23 & -0.18 & -0.43 & -0.41 & -0.39 & -0.08 & -0.06 & -0.14 & -0.09 & -0.22 & -0.07 & -0.39 \\
        DSJR500.5 & 7059.4 & 6738.0 & 1.7 & 1.5 & 27.8 & 242.0 & 1.0 & -0.48 & -0.48 & -0.14 & -0.14 & -0.57 & -0.44 & -0.48 & -0.09 & -0.08 & -0.11 & -0.12 & -0.31 & -0.06 & -0.48 \\
        school1\_nsh & 16043.3 & 2098.6 & 9.3 & 204.8 & 127.7 & 66.5 & 1.0 & -1.31 & -0.82 & -1.44 & -1.42 & -1.44 & -1.0 & -0.49 & -0.36 & -0.11 & -0.8 & -0.44 & -0.7 & -0.19 & -0.49 \\
        flat300\_20\_0 & 5701.5 & 2828.6 & 5.3 & 5.0 & 28.1 & 73.4 & 1.0 & -0.84 & -0.77 & -0.42 & -0.26 & -0.84 & -0.84 & -0.67 & -0.1 & -0.08 & -0.25 & -0.13 & -0.4 & -0.2 & -0.67 \\
        DSJC250.1 & 12482.8 & 1383.2 & 17.0 & 204.7 & 219.0 & 682.3 & 1.0 & -0.65 & -0.32 & -0.68 & -0.69 & -0.7 & -0.5 & -0.35 & -0.28 & -0.06 & -0.42 & -0.15 & -0.31 & -0.09 & -0.35 \\
        queen14\_14 & 4688.3 & 7213.9 & 9.0 & 1615.8 & 22.7 & 61.5 & 1.0 & -0.22 & -0.25 & -0.27 & -0.27 & -0.27 & -0.22 & -0.25 & -0.05 & -0.05 & -0.18 & -0.09 & -0.15 & -0.05 & -0.25 \\
        DSJC250.5 & 2162.5 & 3218.1 & 5.8 & 5.6 & 18.5 & 81.2 & 1.0 & -0.39 & -0.39 & -0.31 & -0.24 & -0.42 & -0.4 & -0.39 & -0.09 & -0.06 & -0.17 & -0.12 & -0.21 & -0.08 & -0.39 \\
        queen13\_13 & 3767.9 & 5989.8 & 8.8 & 1773.2 & 21.2 & 45.1 & 1.0 & -0.23 & -0.24 & -0.27 & -0.27 & -0.27 & -0.24 & -0.24 & -0.05 & -0.05 & -0.18 & -0.08 & -0.14 & -0.06 & -0.24 \\
        DSJR500.1c & 2.1 & 2.1 & 0.0 & 0.0 & 1.5 & 1.1 & 0.2 & -0.42 & -0.42 & -0.04 & 0.0 & -0.42 & -0.42 & -0.07 & -0.29 & -0.29 & -0.04 & 0.0 & -0.32 & -0.39 & -0.07 \\
        1-FullIns\_5 & 2937.1 & 462.6 & 3.5 & 22120.5 & 132.6 & 1784.4 & 0.9 & -1.02 & -0.58 & -1.02 & -1.02 & -1.02 & -1.02 & -0.68 & -0.46 & -0.14 & -0.71 & -0.98 & -0.54 & -0.27 & -0.68 \\
        1-Insertions\_5 & 3485.7 & 902.0 & 4.8 & 30114.7 & 388.1 & 1221.4 & 0.9 & -0.88 & -0.47 & -0.88 & -0.88 & -0.88 & -0.87 & -0.27 & -0.37 & -0.06 & -0.62 & -0.66 & -0.38 & -0.29 & -0.27 \\
        queen12\_12 & 3135.4 & 3682.1 & 7.4 & 1492.7 & 17.7 & 34.5 & 1.0 & -0.23 & -0.23 & -0.25 & -0.25 & -0.25 & -0.22 & -0.22 & -0.05 & -0.05 & -0.16 & -0.07 & -0.13 & -0.05 & -0.22 \\
        2-FullIns\_4 & 5304.7 & 864.5 & 3.2 & 34333.8 & 102.5 & 92.2 & 0.9 & -0.4 & -0.31 & -0.42 & -0.42 & -0.42 & -0.41 & -0.19 & -0.15 & -0.06 & -0.37 & -0.42 & -0.22 & -0.09 & -0.19 \\
        DSJC250.9 & 83.5 & 84.4 & 0.5 & 0.5 & 4.6 & 4.4 & 1.0 & -0.29 & -0.29 & -0.05 & -0.05 & -0.29 & -0.29 & -0.29 & -0.06 & -0.06 & -0.05 & -0.05 & -0.16 & -0.16 & -0.29 \\
        2-Insertions\_4 & 2593.7 & 3703.5 & 4.0 & 38473.6 & 332.6 & 1536.9 & 1.0 & -0.53 & -0.36 & -0.53 & -0.53 & -0.53 & -0.51 & -0.17 & -0.21 & -0.05 & -0.36 & -0.36 & -0.24 & -0.19 & -0.17 \\
        r250.5 & 2692.6 & 3215.2 & 4.6 & 362.4 & 19.4 & 62.6 & 1.0 & -0.47 & -0.49 & -0.54 & -0.54 & -0.54 & -0.4 & -0.4 & -0.12 & -0.12 & -0.31 & -0.21 & -0.29 & -0.11 & -0.4 \\
        queen11\_11 & 2183.0 & 2510.9 & 7.0 & 1692.8 & 14.6 & 22.4 & 1.0 & -0.22 & -0.22 & -0.24 & -0.24 & -0.24 & -0.23 & -0.21 & -0.05 & -0.04 & -0.15 & -0.07 & -0.12 & -0.07 & -0.21 \\
        mug100\_1 & 4005.9 & 5590.3 & 6.4 & 22685.2 & 186.8 & 796.4 & 1.0 & -0.13 & -0.12 & -0.16 & -0.16 & -0.16 & -0.12 & -0.12 & -0.04 & -0.04 & -0.1 & -0.08 & -0.09 & -0.02 & -0.12 \\
        mug100\_25 & 4399.0 & 5410.9 & 6.1 & 23163.2 & 195.2 & 748.5 & 1.0 & -0.14 & -0.13 & -0.16 & -0.16 & -0.16 & -0.13 & -0.12 & -0.05 & -0.04 & -0.1 & -0.09 & -0.09 & -0.02 & -0.12 \\
        mug88\_1 & 3220.0 & 3931.6 & 6.9 & 19528.0 & 146.7 & 117.4 & 1.0 & -0.11 & -0.11 & -0.13 & -0.13 & -0.13 & -0.11 & -0.1 & -0.03 & -0.03 & -0.09 & -0.07 & -0.07 & -0.02 & -0.1 \\
        myciel7 & 820.5 & 192.4 & 3.4 & 32820.8 & 133.6 & 624.0 & 0.7 & -1.53 & -0.89 & -1.53 & -1.53 & -1.53 & -1.47 & -0.27 & -0.45 & -0.13 & -1.1 & -0.96 & -0.48 & -0.37 & -0.27 \\
        DSJC125.1 & 4929.4 & 1644.3 & 11.0 & 35475.4 & 131.7 & 156.2 & 1.0 & -0.5 & -0.32 & -0.51 & -0.51 & -0.51 & -0.43 & -0.23 & -0.2 & -0.07 & -0.29 & -0.41 & -0.23 & -0.09 & -0.23 \\
        mug88\_25 & 3290.2 & 3953.1 & 5.8 & 22046.8 & 144.0 & 431.0 & 1.0 & -0.12 & -0.12 & -0.15 & -0.15 & -0.15 & -0.12 & -0.12 & -0.04 & -0.03 & -0.1 & -0.07 & -0.08 & -0.02 & -0.12 \\
        queen10\_10 & 1194.7 & 1402.9 & 6.0 & 1502.6 & 10.2 & 14.7 & 1.0 & -0.21 & -0.21 & -0.22 & -0.22 & -0.22 & -0.22 & -0.21 & -0.05 & -0.04 & -0.15 & -0.06 & -0.12 & -0.09 & -0.21 \\
        DSJC125.5 & 325.4 & 620.0 & 7.6 & 123.5 & 11.5 & 14.9 & 1.0 & -0.29 & -0.3 & -0.31 & -0.3 & -0.31 & -0.21 & -0.25 & -0.07 & -0.06 & -0.17 & -0.07 & -0.16 & -0.08 & -0.25 \\
        4-Insertions\_3 & 924.6 & 1832.0 & 2.8 & 33978.0 & 87.2 & 425.2 & 0.9 & -0.23 & -0.22 & -0.24 & -0.24 & -0.24 & -0.24 & -0.09 & -0.07 & -0.05 & -0.16 & -0.1 & -0.13 & -0.06 & -0.09 \\
        queen9\_9 & 545.8 & 610.2 & 4.8 & 1744.5 & 9.7 & 8.9 & 1.0 & -0.21 & -0.21 & -0.22 & -0.22 & -0.22 & -0.18 & -0.2 & -0.05 & -0.05 & -0.14 & -0.04 & -0.12 & -0.08 & -0.2 \\
        r125.5 & 425.1 & 757.3 & 3.3 & 3655.7 & 11.5 & 11.4 & 1.0 & -0.39 & -0.4 & -0.4 & -0.4 & -0.4 & -0.4 & -0.31 & -0.14 & -0.15 & -0.29 & -0.13 & -0.24 & -0.2 & -0.31 \\
        DSJC125.9 & 6.8 & 6.8 & 2.3 & 4.7 & 2.8 & 2.0 & 1.0 & -0.19 & -0.19 & -0.19 & -0.19 & -0.19 & -0.19 & -0.19 & -0.08 & -0.08 & -0.14 & -0.1 & -0.12 & -0.14 & -0.19 \\
        1-FullIns\_4 & 213.7 & 110.3 & 2.9 & 41261.2 & 21.1 & 61.1 & 0.8 & -0.29 & -0.26 & -0.29 & -0.29 & -0.29 & -0.29 & -0.17 & -0.12 & -0.08 & -0.19 & -0.21 & -0.16 & -0.11 & -0.17 \\
        1-Insertions\_4 & 180.7 & 297.4 & 5.3 & 23800.0 & 50.8 & 65.0 & 0.9 & -0.23 & -0.21 & -0.23 & -0.23 & -0.23 & -0.21 & -0.08 & -0.06 & -0.04 & -0.16 & -0.06 & -0.09 & -0.06 & -0.08 \\
        myciel6 & 207.7 & 205.0 & 4.0 & 48811.9 & 68.1 & 134.1 & 0.6 & -0.69 & -0.56 & -0.69 & -0.69 & -0.69 & -0.69 & -0.09 & -0.19 & -0.1 & -0.54 & -0.28 & -0.24 & -0.2 & -0.09 \\
        3-Insertions\_3 & 204.4 & 361.5 & 4.0 & 16366.9 & 34.5 & 100.5 & 1.0 & -0.17 & -0.17 & -0.18 & -0.18 & -0.18 & -0.18 & -0.12 & -0.04 & -0.04 & -0.11 & -0.05 & -0.09 & -0.05 & -0.12 \\
        queen8\_8 & 180.3 & 177.8 & 4.1 & 353.2 & 5.0 & 6.9 & 1.0 & -0.17 & -0.17 & -0.17 & -0.17 & -0.17 & -0.17 & -0.16 & -0.04 & -0.04 & -0.12 & -0.03 & -0.1 & -0.09 & -0.16 \\
        2-Insertions\_3 & 26.3 & 29.5 & 3.1 & 177.9 & 5.8 & 5.9 & 1.0 & -0.07 & -0.07 & -0.07 & -0.07 & -0.07 & -0.07 & -0.07 & -0.03 & -0.03 & -0.06 & -0.02 & -0.04 & -0.04 & -0.07 \\
        myciel5 & 34.0 & 41.2 & 3.5 & 1038.7 & 14.6 & 12.8 & 0.8 & -0.28 & -0.27 & -0.28 & -0.28 & -0.28 & -0.28 & -0.13 & -0.1 & -0.08 & -0.21 & -0.04 & -0.11 & -0.09 & -0.13 \\
        myciel4 & 2.6 & 2.7 & 1.2 & 3.3 & 1.4 & 1.2 & 0.8 & -0.09 & -0.09 & -0.09 & -0.09 & -0.09 & -0.09 & -0.09 & -0.06 & -0.06 & -0.08 & -0.06 & -0.07 & -0.08 & -0.09 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/cg/small/table_solving_stats.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccccccccccccccccccccc@{}}
        \toprule
        ash608GPIA & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3.372 & 3.368 & 3.394 & 3.392 & 3.394 & 3.385 & 3.394 & 2045.9 & 1988.8 & 1927.9 & 1887.1 & 1935.3 & 1903.0 & 1963.3 \\
        wap08a & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 47.53 & 62.258 & 58.627 & 57.94 & 65.334 & 65.456 & 64.801 & 2086.6 & 1926.8 & 1906.5 & 1911.9 & 1961.7 & 2043.5 & 1884.0 \\
        wap07a & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 47.105 & 60.4 & 59.423 & 57.184 & 63.366 & 63.496 & 62.555 & 2217.2 & 1959.4 & 2004.6 & 1983.0 & 2057.1 & 1987.6 & 1894.3 \\
        abb313GPIA & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 8.455 & 9.371 & 9.345 & 9.334 & 9.54 & 9.483 & 9.588 & 2164.1 & 1902.6 & 1896.7 & 1904.0 & 1900.3 & 1908.6 & 2154.6 \\
        3-FullIns\_5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 5.697 & 8.763 & 7.684 & 6.648 & 9.672 & 6.607 & 9.349 & 1903.7 & 1866.0 & 1865.7 & 1870.7 & 1866.6 & 1913.2 & 1840.9 \\
        DSJC1000.1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 19.984 & 21.028 & 22.107 & 22.124 & 22.296 & 20.837 & 21.645 & 1890.5 & 1880.8 & 1863.8 & 1866.9 & 1977.2 & 1899.9 & 1851.4 \\
        3-Insertions\_5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3.343 & 4.425 & 3.974 & 3.622 & 4.609 & 3.866 & 4.871 & 1939.7 & 1858.7 & 1852.9 & 1899.9 & 1897.8 & 1915.2 & 1911.4 \\
        r1000.1 & 24 & 24 & 24 & 24 & 11 & 24 & 24 & 20.0 & 20.0 & 20.0 & 20.0 & 20.017 & 20.0 & 20.0 & 210.3 & 263.0 & 145.4 & 224.3 & 1473.1 & 633.1 & 300.2 \\
        DSJC1000.5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 78.028 & 78.401 & 90.751 & 90.786 & 88.568 & 84.175 & 87.938 & 1841.3 & 1869.4 & 1825.2 & 1836.2 & 1850.5 & 1837.6 & 1828.3 \\
        flat1000\_60\_0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 76.308 & 75.755 & 89.235 & 89.272 & 87.034 & 81.522 & 85.709 & 1841.7 & 1867.8 & 1838.2 & 1828.5 & 1851.6 & 1836.4 & 1821.9 \\
        flat1000\_76\_0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 77.293 & 77.134 & 89.58 & 89.589 & 87.434 & 82.189 & 86.803 & 1844.9 & 1861.5 & 1830.5 & 1829.8 & 1835.0 & 1827.9 & 1823.8 \\
        flat1000\_50\_0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 51.76 & 61.696 & 88.794 & 88.788 & 86.42 & 66.964 & 80.768 & 1828.8 & 1845.9 & 1830.5 & 1838.6 & 1850.3 & 1828.0 & 1815.7 \\
        5-FullIns\_4 & 10 & 0 & 0 & 18 & 0 & 0 & 0 & 7.283 & 7.616 & 7.407 & 7.285 & 7.715 & 7.325 & 7.902 & 1584.0 & 1827.4 & 1823.4 & 1567.2 & 2084.8 & 1833.0 & 1807.3 \\
        will199GPIA & 23 & 0 & 5 & 5 & 0 & 0 & 0 & 6.2 & 6.244 & 6.204 & 6.208 & 6.543 & 6.241 & 6.482 & 818.2 & 1833.6 & 1787.0 & 1793.6 & 2171.2 & 1829.5 & 2422.4 \\
        wap05a & 24 & 0 & 24 & 24 & 24 & 0 & 0 & 50.0 & 50.396 & 50.0 & 50.0 & 50.0 & 55.367 & 51.529 & 80.2 & 1837.7 & 426.0 & 365.7 & 435.4 & 1829.1 & 1812.5 \\
        wap06a & 12 & 0 & 0 & 0 & 0 & 0 & 0 & 40.012 & 51.262 & 43.622 & 43.47 & 42.989 & 56.945 & 53.552 & 1770.2 & 1825.1 & 1823.2 & 1841.5 & 1868.6 & 1816.9 & 1811.4 \\
        DSJC1000.9 & 24 & 24 & 0 & 0 & 24 & 0 & 0 & 214.855 & 214.855 & 228.839 & 228.876 & 214.855 & 214.973 & 219.215 & 274.1 & 372.9 & 1813.4 & 1831.6 & 1579.4 & 1806.1 & 1805.1 \\
        DSJC500.1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 11.415 & 12.141 & 12.8 & 12.93 & 13.394 & 11.363 & 11.848 & 1811.2 & 1819.3 & 1821.5 & 1813.1 & 2020.6 & 1824.9 & 1815.7 \\
        2-FullIns\_5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 4.737 & 5.61 & 5.247 & 4.829 & 5.593 & 4.973 & 6.105 & 1825.7 & 1820.2 & 1810.8 & 1832.4 & 1845.6 & 1822.9 & 1803.5 \\
        4-Insertions\_4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2.592 & 2.745 & 2.852 & 2.777 & 3.124 & 2.641 & 3.025 & 1821.2 & 1820.1 & 1809.2 & 1833.7 & 1836.5 & 1832.5 & 1803.5 \\
        2-Insertions\_5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2.92 & 3.458 & 3.349 & 3.22 & 3.73 & 2.978 & 3.747 & 1856.7 & 1823.3 & 1813.4 & 1834.1 & 1828.5 & 1841.8 & 1803.4 \\
        4-FullIns\_4 & 24 & 0 & 24 & 17 & 0 & 22 & 0 & 6.329 & 6.389 & 6.329 & 6.33 & 6.432 & 6.329 & 6.575 & 636.0 & 1817.5 & 778.0 & 1605.9 & 1922.9 & 1099.2 & 1803.2 \\
        r1000.5 & 14 & 24 & 0 & 0 & 24 & 0 & 0 & 234.053 & 234.0 & 268.258 & 268.283 & 234.0 & 249.398 & 243.494 & 1590.5 & 1155.1 & 1820.8 & 1819.0 & 786.8 & 1816.5 & 1803.1 \\
        DSJC500.5 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 42.453 & 42.628 & 50.549 & 50.607 & 42.347 & 43.559 & 44.098 & 1804.5 & 1815.7 & 1815.8 & 1815.3 & 1808.1 & 1805.3 & 1801.8 \\
        1-Insertions\_6 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3.227 & 4.264 & 3.918 & 3.757 & 4.029 & 3.324 & 4.664 & 1830.3 & 1820.3 & 1815.1 & 1821.4 & 1830.1 & 1822.5 & 1802.1 \\
        le450\_5a & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 6.247 & 6.031 & 7.017 & 6.927 & 8.88 & 6.129 & 7.336 & 1813.9 & 1816.9 & 1820.0 & 1820.5 & 1936.5 & 1818.7 & 1801.9 \\
        le450\_5b & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 6.299 & 5.9 & 7.025 & 6.938 & 8.837 & 6.113 & 7.321 & 1810.6 & 1820.3 & 1822.0 & 1824.6 & 1910.7 & 1830.5 & 1802.1 \\
        r1000.1c & 24 & 24 & 0 & 0 & 24 & 24 & 1 & 95.057 & 95.057 & 95.197 & 95.2 & 95.057 & 95.057 & 95.071 & 21.5 & 128.8 & 1828.0 & 1828.6 & 68.7 & 53.2 & 1800.3 \\
        le450\_25a & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 25.0 & 25.0 & 25.0 & 25.0 & 25.0 & 25.0 & 25.0 & 11.4 & 90.8 & 11.5 & 155.0 & 10.5 & 637.3 & 98.3 \\
        le450\_15d & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 17.725 & 21.902 & 20.015 & 19.318 & 21.687 & 21.862 & 21.212 & 1807.4 & 1822.9 & 1826.7 & 1813.2 & 1822.8 & 1812.7 & 1802.7 \\
        le450\_15c & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 17.553 & 21.913 & 20.061 & 19.304 & 21.458 & 21.734 & 21.002 & 1807.3 & 1816.0 & 1821.7 & 1812.8 & 1826.6 & 1811.5 & 1802.8 \\
        le450\_15b & 24 & 0 & 24 & 24 & 0 & 0 & 0 & 15.0 & 17.082 & 15.0 & 15.0 & 15.932 & 17.327 & 15.921 & 109.4 & 1816.1 & 1265.6 & 970.5 & 1895.9 & 1814.9 & 1802.2 \\
        le450\_15a & 24 & 0 & 24 & 24 & 0 & 0 & 0 & 15.0 & 17.186 & 15.0 & 15.0 & 15.87 & 17.557 & 15.941 & 127.6 & 1820.1 & 1319.0 & 977.5 & 1872.4 & 1812.1 & 1801.6 \\
        le450\_25c & 24 & 0 & 0 & 0 & 0 & 0 & 0 & 25.0 & 28.468 & 25.428 & 25.166 & 25.942 & 29.577 & 27.268 & 254.0 & 1818.9 & 1812.3 & 1827.4 & 1827.5 & 1810.2 & 1800.8 \\
        le450\_25d & 24 & 0 & 0 & 0 & 0 & 0 & 0 & 25.0 & 28.011 & 25.408 & 25.136 & 26.091 & 29.055 & 27.246 & 188.5 & 1820.2 & 1807.9 & 1824.6 & 1826.7 & 1812.9 & 1801.2 \\
        le450\_5c & 0 & 7 & 0 & 0 & 0 & 0 & 0 & 5.346 & 5.109 & 7.423 & 7.112 & 7.477 & 5.44 & 7.071 & 1805.3 & 1462.8 & 1819.5 & 1815.1 & 1821.3 & 1817.6 & 1803.4 \\
        queen16\_16 & 24 & 24 & 24 & 24 & 0 & 17 & 24 & 16.0 & 16.0 & 16.0 & 16.0 & 16.805 & 16.07 & 16.0 & 34.8 & 135.0 & 418.2 & 506.5 & 1818.5 & 830.4 & 697.8 \\
        le450\_5d & 0 & 11 & 0 & 0 & 0 & 0 & 0 & 5.343 & 5.092 & 7.395 & 6.997 & 7.565 & 5.351 & 7.037 & 1808.1 & 1311.5 & 1816.8 & 1816.6 & 1823.0 & 1814.0 & 1805.4 \\
        DSJC500.9 & 24 & 24 & 0 & 0 & 24 & 24 & 24 & 122.306 & 122.306 & 125.304 & 125.23 & 122.306 & 122.306 & 122.306 & 12.6 & 168.4 & 1824.1 & 1827.0 & 71.7 & 111.6 & 389.0 \\
        3-FullIns\_4 & 24 & 24 & 24 & 24 & 24 & 24 & 23 & 5.392 & 5.392 & 5.392 & 5.392 & 5.392 & 5.392 & 5.392 & 49.4 & 533.3 & 119.7 & 789.1 & 327.7 & 220.2 & 704.6 \\
        3-Insertions\_4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2.533 & 2.619 & 2.604 & 2.715 & 2.79 & 2.477 & 2.796 & 1813.8 & 1818.3 & 1805.0 & 1819.6 & 1819.9 & 1811.3 & 1801.1 \\
        queen15\_15 & 24 & 24 & 24 & 24 & 0 & 22 & 24 & 15.0 & 15.0 & 15.0 & 15.0 & 15.326 & 15.092 & 15.0 & 18.9 & 58.1 & 269.0 & 399.8 & 1824.6 & 319.0 & 373.8 \\
        school1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 15.42 & 21.96 & 19.523 & 18.627 & 15.87 & 16.188 & 18.333 & 1804.1 & 1811.1 & 1813.0 & 1819.1 & 1803.1 & 1804.7 & 1800.6 \\
        flat300\_26\_0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 26.0 & 26.0 & 30.654 & 31.302 & 26.0 & 26.254 & 26.0 & 1802.6 & 1806.8 & 1828.8 & 1816.9 & 1801.6 & 1800.8 & 1800.4 \\
        flat300\_28\_0 & 0 & 9 & 0 & 0 & 24 & 19 & 3 & 27.525 & 27.52 & 30.78 & 31.266 & 27.52 & 27.698 & 27.52 & 1801.1 & 1678.0 & 1828.0 & 1818.7 & 225.0 & 1203.9 & 1761.4 \\
        DSJR500.5 & 24 & 24 & 0 & 0 & 24 & 21 & 24 & 122.0 & 122.0 & 132.687 & 132.97 & 122.0 & 122.399 & 122.0 & 16.4 & 159.8 & 1810.8 & 1807.6 & 38.9 & 677.9 & 274.4 \\
        school1\_nsh & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 15.657 & 21.559 & 18.142 & 17.589 & 15.176 & 17.25 & 17.854 & 1803.1 & 1810.7 & 1814.7 & 1811.4 & 1802.8 & 1802.8 & 1800.6 \\
        flat300\_20\_0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 20.0 & 20.0 & 24.526 & 29.374 & 20.522 & 20.0 & 20.896 & 1802.9 & 1806.1 & 1816.7 & 1824.8 & 1801.5 & 1801.8 & 1800.4 \\
        DSJC250.1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 7.079 & 7.625 & 7.466 & 7.499 & 8.033 & 7.004 & 7.33 & 1973.5 & 1817.1 & 1813.0 & 1808.8 & 1821.8 & 1804.5 & 1833.9 \\
        queen14\_14 & 24 & 24 & 24 & 24 & 24 & 23 & 24 & 14.0 & 14.0 & 14.0 & 14.0 & 14.0 & 14.017 & 14.0 & 12.1 & 31.2 & 183.7 & 343.4 & 220.1 & 235.0 & 218.8 \\
        DSJC250.5 & 5 & 24 & 0 & 0 & 24 & 24 & 17 & 25.166 & 25.165 & 26.714 & 27.118 & 25.165 & 25.165 & 25.165 & 1746.4 & 310.4 & 1816.2 & 1807.5 & 83.9 & 302.2 & 1240.2 \\
        queen13\_13 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 13.0 & 13.0 & 13.0 & 13.0 & 13.0 & 13.0 & 13.0 & 5.5 & 13.4 & 91.3 & 245.5 & 42.9 & 47.0 & 104.8 \\
        DSJR500.1c & 24 & 24 & 11 & 13 & 24 & 24 & 24 & 84.136 & 84.136 & 84.158 & 84.161 & 84.136 & 84.136 & 84.136 & 1.8 & 62.2 & 1152.5 & 1171.6 & 1.2 & 1.4 & 26.5 \\
        1-FullIns\_5 & 24 & 1 & 15 & 0 & 0 & 24 & 0 & 3.909 & 3.957 & 3.91 & 3.933 & 3.939 & 3.909 & 3.974 & 13.0 & 1777.8 & 1581.4 & 1813.2 & 1808.5 & 118.7 & 1800.3 \\
        1-Insertions\_5 & 0 & 0 & 0 & 0 & 0 & 24 & 0 & 2.953 & 3.13 & 2.963 & 3.11 & 2.988 & 2.943 & 3.149 & 1801.5 & 1813.2 & 1803.2 & 1816.7 & 1803.8 & 449.8 & 1800.4 \\
        queen12\_12 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 12.0 & 12.0 & 12.0 & 12.0 & 12.0 & 12.0 & 12.0 & 3.4 & 7.2 & 60.2 & 217.4 & 13.3 & 29.1 & 60.3 \\
        2-FullIns\_4 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 4.485 & 4.485 & 4.485 & 4.485 & 4.485 & 4.485 & 4.485 & 4.0 & 157.3 & 14.0 & 391.5 & 15.6 & 17.9 & 298.0 \\
        DSJC250.9 & 24 & 24 & 0 & 0 & 24 & 24 & 24 & 70.392 & 70.392 & 71.24 & 71.242 & 70.392 & 70.392 & 70.392 & 1.5 & 6.2 & 1833.7 & 1836.3 & 4.9 & 6.5 & 16.4 \\
        2-Insertions\_4 & 0 & 0 & 24 & 0 & 24 & 24 & 0 & 2.567 & 2.592 & 2.56 & 2.671 & 2.56 & 2.56 & 2.6 & 1801.0 & 1803.1 & 439.7 & 1805.8 & 1328.3 & 239.0 & 1800.5 \\
        r250.5 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 65.0 & 65.0 & 65.0 & 65.0 & 65.0 & 65.0 & 65.0 & 2.2 & 11.3 & 476.3 & 282.3 & 4.3 & 61.4 & 26.1 \\
        queen11\_11 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 11.0 & 11.0 & 11.0 & 11.0 & 11.0 & 11.0 & 11.0 & 2.0 & 3.6 & 36.3 & 182.5 & 5.9 & 14.5 & 32.0 \\
        mug100\_1 & 24 & 24 & 24 & 0 & 24 & 24 & 24 & 3.03 & 3.03 & 3.03 & 3.044 & 3.03 & 3.03 & 3.03 & 9.5 & 27.5 & 17.5 & 1811.1 & 18.6 & 54.8 & 48.3 \\
        mug100\_25 & 24 & 24 & 24 & 2 & 24 & 24 & 24 & 3.03 & 3.03 & 3.03 & 3.036 & 3.03 & 3.03 & 3.03 & 6.6 & 21.6 & 16.4 & 1809.1 & 15.8 & 48.8 & 42.6 \\
        mug88\_1 & 24 & 24 & 24 & 14 & 24 & 24 & 24 & 3.034 & 3.034 & 3.034 & 3.036 & 3.034 & 3.034 & 3.034 & 3.4 & 9.3 & 8.7 & 1640.1 & 6.5 & 25.7 & 18.8 \\
        myciel7 & 24 & 0 & 24 & 0 & 9 & 24 & 0 & 4.095 & 4.16 & 4.095 & 4.212 & 4.113 & 4.095 & 4.097 & 132.8 & 1807.9 & 1097.1 & 1807.6 & 1625.9 & 124.2 & 1800.2 \\
        DSJC125.1 & 0 & 0 & 24 & 0 & 24 & 0 & 0 & 4.458 & 4.565 & 4.454 & 4.47 & 4.454 & 4.484 & 4.461 & 1800.3 & 1801.1 & 495.2 & 1808.7 & 75.2 & 1800.6 & 1800.2 \\
        mug88\_25 & 24 & 24 & 24 & 5 & 24 & 24 & 24 & 3.034 & 3.034 & 3.034 & 3.038 & 3.034 & 3.034 & 3.034 & 3.9 & 9.3 & 9.4 & 1761.2 & 8.1 & 23.1 & 22.6 \\
        queen10\_10 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 1.2 & 1.7 & 28.1 & 158.2 & 3.7 & 8.4 & 21.1 \\
        DSJC125.5 & 24 & 24 & 24 & 6 & 24 & 24 & 24 & 15.727 & 15.727 & 15.727 & 15.727 & 15.727 & 15.727 & 15.727 & 56.2 & 7.8 & 908.7 & 1607.6 & 4.8 & 14.3 & 53.5 \\
        4-Insertions\_3 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 2.276 & 2.276 & 2.276 & 2.276 & 2.276 & 2.276 & 2.276 & 362.8 & 299.8 & 16.7 & 882.1 & 8.8 & 25.6 & 61.5 \\
        queen9\_9 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 9.0 & 9.0 & 9.0 & 9.0 & 9.0 & 9.0 & 9.0 & 0.5 & 0.7 & 9.8 & 132.9 & 1.4 & 3.5 & 7.0 \\
        r125.5 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 36.0 & 36.0 & 36.0 & 36.0 & 36.0 & 36.0 & 36.0 & 0.3 & 0.7 & 3.5 & 77.8 & 0.3 & 1.0 & 1.2 \\
        DSJC125.9 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 42.727 & 42.727 & 42.727 & 42.727 & 42.727 & 42.727 & 42.727 & 0.2 & 0.5 & 53.7 & 115.4 & 0.3 & 0.4 & 0.5 \\
        1-FullIns\_4 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 3.633 & 3.633 & 3.633 & 3.633 & 3.633 & 3.633 & 3.633 & 0.2 & 1.3 & 2.0 & 71.0 & 0.9 & 0.7 & 1.4 \\
        1-Insertions\_4 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 2.774 & 2.774 & 2.774 & 2.774 & 2.774 & 2.774 & 2.774 & 3.3 & 39.0 & 9.2 & 484.7 & 2.4 & 4.5 & 19.2 \\
        myciel6 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 3.834 & 3.834 & 3.834 & 3.834 & 3.834 & 3.834 & 3.834 & 1.9 & 518.7 & 28.6 & 794.1 & 12.1 & 9.9 & 76.1 \\
        3-Insertions\_3 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 2.334 & 2.334 & 2.334 & 2.334 & 2.334 & 2.334 & 2.334 & 6.8 & 13.2 & 3.5 & 300.1 & 1.1 & 4.1 & 11.2 \\
        queen8\_8 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 8.444 & 8.444 & 8.444 & 8.444 & 8.444 & 8.444 & 8.444 & 0.1 & 0.1 & 1.3 & 60.1 & 0.2 & 0.4 & 0.4 \\
        2-Insertions\_3 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 2.423 & 2.423 & 2.423 & 2.423 & 2.423 & 2.423 & 2.423 & 0.2 & 0.3 & 0.6 & 112.8 & 0.2 & 0.4 & 0.4 \\
        myciel5 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 3.553 & 3.553 & 3.553 & 3.553 & 3.553 & 3.553 & 3.553 & 0.1 & 1.2 & 1.1 & 139.0 & 0.3 & 0.7 & 1.6 \\
        myciel4 & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 3.245 & 3.245 & 3.245 & 3.245 & 3.245 & 3.245 & 3.245 & 0.0 & 0.0 & 0.1 & 2.2 & 0.0 & 0.0 & 0.0 \\
        statistic & 1096 & 916 & 895 & 728 & 932 & 964 & 812 & 12.934 & 13.615 & 13.838 & 13.78 & 13.903 & 13.494 & 13.926 & 125.6 & 253.7 & 355.2 & 899.0 & 199.2 & 244.7 & 350.1 \\
        \bottomrule
    \end{tabular}
\end{table}


==> data/table_graph.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}cccc@{}}
        \toprule
        4-FullIns\_5 & 4146 & 0.009 & 1280.5 \\
        ash958GPIA & 1916 & 0.007 & 938.8 \\
        wap02a & 2464 & 0.037 & 821.4 \\
        C2000.5 & 2000 & 0.5 & 648.7 \\
        wap01a & 2368 & 0.04 & 582.6 \\
        wap08a & 1870 & 0.06 & 234.2 \\
        ash608GPIA & 1216 & 0.011 & 232.7 \\
        wap07a & 1809 & 0.063 & 230.9 \\
        abb313GPIA & 1557 & 0.054 & 161.7 \\
        3-FullIns\_5 & 2030 & 0.016 & 133.8 \\
        DSJC1000.1 & 1000 & 0.099 & 113.5 \\
        3-Insertions\_5 & 1406 & 0.01 & 98.8 \\
        r1000.1 & 1000 & 0.029 & 61.1 \\
        DSJC1000.5 & 1000 & 0.5 & 57.2 \\
        flat1000\_60\_0 & 1000 & 0.492 & 55.4 \\
        flat1000\_76\_0 & 1000 & 0.494 & 55.1 \\
        flat1000\_50\_0 & 1000 & 0.49 & 53.4 \\
        5-FullIns\_4 & 1085 & 0.019 & 30.2 \\
        will199GPIA & 701 & 0.029 & 22.4 \\
        wap05a & 905 & 0.105 & 21.8 \\
        wap06a & 947 & 0.097 & 21.3 \\
        DSJC1000.9 & 1000 & 0.9 & 10.2 \\
        DSJC500.1 & 500 & 0.1 & 8.4 \\
        2-FullIns\_5 & 852 & 0.034 & 7.7 \\
        4-Insertions\_4 & 475 & 0.016 & 6.9 \\
        2-Insertions\_5 & 597 & 0.022 & 6.1 \\
        4-FullIns\_4 & 690 & 0.028 & 5.6 \\
        r1000.5 & 1000 & 0.477 & 5.6 \\
        DSJC500.5 & 500 & 0.502 & 5.1 \\
        1-Insertions\_6 & 607 & 0.034 & 4.9 \\
        le450\_5a & 450 & 0.057 & 4.5 \\
        le450\_5b & 450 & 0.057 & 4.3 \\
        r1000.1c & 1000 & 0.971 & 3.0 \\
        le450\_25a & 450 & 0.082 & 2.8 \\
        le450\_15d & 450 & 0.166 & 2.6 \\
        le450\_15c & 450 & 0.165 & 2.6 \\
        le450\_15b & 450 & 0.081 & 2.3 \\
        le450\_15a & 450 & 0.081 & 2.3 \\
        le450\_25c & 450 & 0.172 & 2.1 \\
        le450\_25d & 450 & 0.172 & 2.1 \\
        le450\_5c & 450 & 0.097 & 1.8 \\
        queen16\_16 & 256 & 0.387 & 1.8 \\
        le450\_5d & 450 & 0.097 & 1.8 \\
        DSJC500.9 & 500 & 0.901 & 1.4 \\
        3-FullIns\_4 & 405 & 0.043 & 1.3 \\
        queen15\_15 & 225 & 0.411 & 1.2 \\
        3-Insertions\_4 & 281 & 0.027 & 1.2 \\
        school1 & 385 & 0.258 & 1.1 \\
        DSJR500.5 & 500 & 0.472 & 1.1 \\
        flat300\_26\_0 & 300 & 0.482 & 1.1 \\
        flat300\_28\_0 & 300 & 0.484 & 1.1 \\
        school1\_nsh & 352 & 0.237 & 1.1 \\
        flat300\_20\_0 & 300 & 0.477 & 1.0 \\
        DSJC250.1 & 250 & 0.103 & 0.8 \\
        queen14\_14 & 196 & 0.438 & 0.8 \\
        DSJC250.5 & 250 & 0.503 & 0.6 \\
        queen13\_13 & 169 & 0.469 & 0.5 \\
        DSJR500.1c & 500 & 0.972 & 0.5 \\
        1-FullIns\_5 & 282 & 0.082 & 0.4 \\
        1-Insertions\_5 & 202 & 0.06 & 0.4 \\
        queen12\_12 & 144 & 0.504 & 0.3 \\
        2-FullIns\_4 & 212 & 0.072 & 0.3 \\
        DSJC250.9 & 250 & 0.896 & 0.2 \\
        2-Insertions\_4 & 149 & 0.049 & 0.2 \\
        r250.5 & 250 & 0.477 & 0.2 \\
        queen11\_11 & 121 & 0.545 & 0.2 \\
        mug100\_1 & 100 & 0.034 & 0.2 \\
        mug100\_25 & 100 & 0.034 & 0.2 \\
        mug88\_1 & 88 & 0.038 & 0.1 \\
        myciel7 & 191 & 0.13 & 0.1 \\
        DSJC125.1 & 125 & 0.095 & 0.1 \\
        mug88\_25 & 88 & 0.038 & 0.1 \\
        queen10\_10 & 100 & 0.594 & 0.1 \\
        DSJC125.5 & 125 & 0.502 & 0.1 \\
        4-Insertions\_3 & 79 & 0.051 & 0.1 \\
        queen9\_9 & 81 & 0.652 & 0.1 \\
        r125.5 & 125 & 0.495 & 0.1 \\
        DSJC125.9 & 125 & 0.898 & 0.0 \\
        1-FullIns\_4 & 93 & 0.139 & 0.0 \\
        1-Insertions\_4 & 67 & 0.105 & 0.0 \\
        myciel6 & 95 & 0.169 & 0.0 \\
        3-Insertions\_3 & 56 & 0.071 & 0.0 \\
        queen8\_8 & 64 & 0.722 & 0.0 \\
        2-Insertions\_3 & 37 & 0.108 & 0.0 \\
        myciel5 & 47 & 0.218 & 0.0 \\
        myciel4 & 23 & 0.281 & 0.0 \\
        \bottomrule
    \end{tabular}
\end{table}

